Physical expander in Virtual Tree Overlay

In this paper, we propose a new construction of constantdegree expanders motivated by their application in P2P overlay networks and in particular in the design of robust trees overlay. Our key result can be stated as follows. Consider a complete binary tree T and construct a random pairing {\Pi} between leaf nodes and internal nodes. We prove that the graph G\Pi obtained from T by contracting all pairs (leaf-internal nodes) achieves a constant node expansion with high probability. The use of our result in improving the robustness of tree overlays is straightforward. That is, if each physical node participating to the overlay manages a random pair that couples one virtual internal node and one virtual leaf node then the physical-node layer exhibits a constant expansion with high probability. We encompass the difficulty of obtaining this random tree virtualization by proposing a local, selforganizing and churn resilient uniformly-random pairing algorithm with O(log2 n) running time. Our algorithm has the merit to not modify the original tree virtual overlay (we just control the mapping between physical nodes and virtual nodes). Therefore, our scheme is general and can be applied to a large number of tree overlay implementations. We validate its performances in dynamic environments via extensive simulations.

==> introduction-old.tex <==
\section{Introduction}

\subsection{Background}
P2P networks are appealing for sharing/diffusing/searching resources among 
heterogeneous groups of users. Efficiently organizing users in order 
to achieve these goals was the main concern that motivated the study 
of overlay networks. In particular, tree overlays are one of attractive
schemes because of its simplicity and rich resources from the 
long history of its study. Many distributed applications or 
communication primitives in P2P networks such as multicast or 
publish/subscribe are tied to the hierarchical and acyclic structure 
of trees\cite{CK09,1009738,EGHKK03,CDKNRS03}. Therefore, it is 
a challenging problem to explore the efficient design of tree overlays 
which offer good searchability and load balancing performances. Many 
P2P and distributed variants of classical tree structures such as 
B-trees, R-trees or P-trees have been designed 
\cite{BATON,VBI,PGrid,Caron06,DRTree,Brushwood}. 

Because of the dynamic nature of P2P networks, robustness 
to faults and churn (e.g., frequent node join and leave) is 
indispensable for the service on the top of them to function properly. 
A recent trend for measuring that kind of 
robustness is the use of {\em graph expansion}. The (node) expansion
$h(G)$ of an undirected graph $G = (V_G, E_G)$ is defined as:
\[
h(G) = \min_{S \subseteq V_G | |S| \leq n/2} \frac{|\nodeboundary{S}|}{|S|},
\]
where $\nodeboundary{S}$ is the set of nodes that are adjacent to a node in 
$S$ but not contained in $S$. The implication of node expansion is that 
deletion of at least $h(G) \cdot k$ nodes is necessary to disconnect a component of $k$ nodes from $G$. That is, we can say that graphs with good expansion 
are hard to be partitioned into a number of large connected components. 
In this sense, the expansion of a graph can be seen as a good measurement 
of fault-tolerance. However, the expansion of tree overlays is trivially
$\Omega(1/n)$, which is far from adequate. This weakness to faults and
churn is the primary reason why tree overlays are not so pervasive in real
applications. 

\subsection{Our Contribution}

Our focus in this paper is to provide the mechanism to make
tree overlays robust. In particular, we are interested in {\em generic}
schemes applicable a large class of tree overlays: As seen above, 
there are many variations of tree-based data structures with 
distinguished characteristics, but their distributed implementations 
always face the problem how to circumvent the threat of disconnection.
Therefore, providing such a generic robustization scheme 
would offer the substantial benefit for implementing distributed
tree-based data structures in a systematic way.

To attain our goal, we look at a novel approach, which we call
{\em tree virtualization}. The principle of tree virtualization is 
very simple: Regarding the tree overlay as a virtual network, one 
physical node is in charge of several virtual nodes constituting 
the tree. Then, the physical-node layer forms a topological 
structures which is expected to be more robust than trees. The 
core of our approach is to explore the mapping from virtual to physical 
such that the physical-node layer exhibits a good robustness 
property. It is notable that tree virtualization schemes are 
independent of the original design of tree overlays. That is, 
since we only control the mapping to physical nodes and do not 
modify the original tree-overaly algorithm. the design scheme
can be applied to a large class of tree-overlay algorithms. 

Our primary contribution is to show the following theorem 
which takes an important role in the above context:
\begin{theorem} \label{thmExpansion}
Let $T$ be a complete $n$-node binary tree with duplication of the 
root node (the duplicated root is seen to be identical to
the original root). Then, we can define a bijective function 
$\Pi$ from leaf nodes to internal nodes. Let $G_\Pi$ be the 
graph obtained from $T$ by contracting pair $(v, \Pi(v))$ for 
all $v$ \footnote{The contraction of $(v, \Pi(v))$ means that we 
contract edge $\{v, \Pi(v)\}$ as if it exists in $T$.}. 
Choosing $\Pi$ uniformly at random (from $(n/2)!$ possible choices), 
$G_\Pi$ has a constant (node) expansion with high probability.
\end{theorem}

The implication of this theorem is that if we assign a random pair of 
one leaf and one internal node to each physical node, the physical-node 
layer achieves a constant expansion with high probability. Given 
that the expansion of tree overlay is the asymptotically smallest 
of all connected graphs, this improvement is surprisingly large.

The above result relies on the uniform random matching between internal 
and leaf nodes in the tree overlay, which is necessary to determine the
mapping of virtual nodes to physicals. Therefore, we also consider 
how to construct the random perfect bipartite matching over
internal and leaf nodes. Fortunately, we can point out that it
is easily constructed in distributed and self-$\ast$ fashion. 
Following the parallel random permutation algorithm by 
Czumaj et. al.\cite{CK00}, we can increase the graph expansion 
to a constant within $O(\log^2 n)$ synchronous rounds ($n$ is 
the number of physical nodes). Since that analysis is the result 
in static environments, we also propose the empirical evaluation of 
our approach in dynamic environments via simulation. The simulation
result present shows that the quick convergence to the constant
expansion still holds in dynamic systems, which justifies the practical
impact of our scheme.

%A straightforward approach to improve the robustness is the construction
%of highly-connected topological structures based on trees by augmenting
%several overlay links. However, since most of tree-based 
%structures rely on their own maintenance mechanisms (i.e., the 
%algorithm of adding or deleting nodes) that are designed in ad-hoc manners, 
%and thus it is hard to install link augmentation schemes to them in 



==> introduction-old2.tex <==
\section{Introduction}

In this paper, we propose a new construction
of constant-degree expanders motibated by an application in distrbitued 
computing. The primary result presented in this paper is stated as
follows: Let $T = (V, E)$ be a complete binary tree with duplication
of the root node (the duplicated root is seen to be identical to
the original root). Then, in $T$, the number of internal nodes 
is equal to the number of leaf nodes, and thus we can define
a bijective function $\Pi$ from leaf nodes to internal nodes. 
Letting $G_\Pi$ be the graph obtained from $T$ by contracting
pair $(v, \Pi(v))$ for all $v$ \footnote{The contraction of 
$(v, \Pi(v))$ means that we contract edge $\{v, \Pi(v)\}$ as if 
it exists in $T$.}, the following theorem holds: 
\begin{theorem} \label{thmExpansion}
Choosing $\Pi$ uniformly at random (from $(|V|/2)!$ possible choices), 
$G_\Pi$ has a constant (node) expansion with high probability.
\end{theorem}
In the remaining part of the introduction, we explain what role this theorem
takes in the context of distributed computing.

\paragraph{Background}
P2P networks are appealing for sharing/diffusing/searching resources among 
heterogeneous groups of users. Efficiently organizing users in order 
to achieve these goals was the main concern that motivated the study 
of overlay networks. In particular, tree overlays are one of attractive
schemes because of its simplicity and rich resources from the 
long history of its study. Many distributed applications or 
communication primitives in P2P networks such as multicast or 
publish/subscribe are tied to the hierarchical and acyclic structure 
of trees\cite{CK09,1009738,EGHKK03,CDKNRS03}.
Therefore, it is a challenging problem to explore the efficient 
design of tree overlays which offer good searchability and load balancing 
performances. Many P2P and distributed variants of classical tree 
structure such as B-trees, R-trees or P-trees have been designed 
\cite{BATON,VBI,PGrid,Caron06,DRTree,Brushwood}. 

Because of the dynamic nature of P2P networks, robustness 
to faults and churn (e.g., frequent node join and leave) is 
indispensable for the service on the top of them to function properly. 
A recent trend for measuring that kind of 
robustness is the use of {\em graph expansion}.
The (node) expansion $h(G)$ of an undirected graph $G = (V_G, E_G)$ is 
defined as:
\[
h(G) = \min_{S \subseteq V_G | |S| \leq n/2} \frac{|\nodeboundary{S}|}{|S|},
\]
where $\nodeboundary{S}$ is the set of nodes that are adjacent to a node in 
$S$ but not contained in $S$. The implication of node expansion is that 
deletion of at least $h(G) \cdot k$ nodes is necessary to disconnect a 
component of $k$ nodes from $G$. That is, we can say that graphs with good
expansion are hard to be partitioned into a number of large connected 
components. 
In this sense, the expansion of a graph can be seen as a good measurement 
of fault-tolerance. However, the expansion of tree overlays is trivially
$\Omega(1/n)$, which is far from adequate. This weakness to faults and
churn is the primary reason why tree overlays are not so pervasive in real
applications. 

\paragraph{Our Contribution}

Our focus in this paper is to provide the mechanism to make
tree overlays robust. In particular, we are interested in {\em generic}
schemes applicable a large class of tree overlays: As seen above, 
there are many variations of tree-based data structures with 
distinguished characteristics, but their distributed implementations 
always face the problem how to circumvent the threat of disconnection.
Therefore, providing such a generic robustization scheme 
would offer the substantial benefit for implementing distributed
tree-based data structures in a systematic way.

A straightforward approach to improve the robustness is the construction
of highly-connected topological structures by augmenting links. However, 
since the maintenance algorithms of tree-based structures 
(i.e., algorithms of adding or deleting nodes) are designed in ad-hoc manners, 
it is hard to design generic link augmentation schemes. Therefore, 
we look at a quite different approach, which we call 
{\em tree virtualization}. The principle of tree virtualization 
is very simple: Regarding the tree overlay as a
virtual network, one physical node is in charge of several 
virtual nodes constituting the tree. Then, the physical-node layer forms
a topological structures which is expected to be more robust than
trees. In that context, we can interpret Therem \ref{thmExpansion} as
follows: If we assign a random pair of one leaf and one internal node to 
each physical node, the physical-node layer has a constant expansion
with high probability. Given that the expansion of tree overlay is 
the asymptotically smallest of all connected graphs, 
this improvement is surprisingly large. Furthermre it is notable that 
our robustization scheme is independent of the original design of tree 
overlays. That is, we only control the mapping to physical nodes and 
do not modify the original tree-overaly algorithm. Because of this 
feature, we can use our scheme combined with any
balanced-tree overlay algorithm. 

In addition to our primary result, we point out that 
our form of random perfect bipartite matchings is easily 
constructed in distributed and self-$\ast$ fashion. Following the 
parallel random permutation algorithm by Czumaj et. al.\cite{CK00}, 
we can obtain a distributed algorithm to obtain the random perfect 
bipartite matching on trees running within $O(\log^2 n)$ 
synchronous rounds. Since that algorithm has the theoretical 
guarantee only in static environments, we also evaluate that algorithm
in dynamic environments via simulation. The simulation result shows 
that the quick convergence to the constant expansion still holds 
in dynamic systems, which justifies the practical impact of our scheme.

\paragraph{Roadmap}
In Section \ref{secRelated}, we introduce the relate work mainly in the field
of distributed computing. Section \ref{secMain} presents the proof of our
main result. The issue about the distributed implmentation of our scheme
is explained in Secton \ref{secDistributed} which includes the simulation 
result. Finally, Section 
\ref{secConclusion} provides the conclusion and future research issues.


